Distributed AI Platform for the 6G RAN

Cellular Radio Access Networks (RANs) are rapidly evolving towards 6G, driven by the need to reduce costs and introduce new revenue streams for operators and enterprises. In this context, AI emerges as a key enabler in solving complex RAN problems spanning both the management and application domains. Unfortunately, and despite the undeniable promise of AI, several practical challenges still remain, hindering the widespread adoption of AI applications in the RAN space. In this work, we attempt to shed light to these challenges and argue that existing approaches in addressing them are inadequate for realizing the vision of a truly AI-native 6G network. We propose a distributed AI platform architecture, tailored to the needs of an AI-native RAN.

==> ai_ran.tex <==
\section{The Need for AI in RAN}
\label{sec:need-for-AI}
Here, we discuss why the need for AI in the RAN space is becoming increasingly important. 
%This need is linked to challenges and opportunities spanning different and heterogeneous aspects of the RAN, from fundamental wireless challenges that have been in the spotlight since the early days of cellular communications, to emerging challenges and opportunities that are related to recent trends in the telecommunications space.
The AI-RAN Alliance has succinctly grouped AI use cases in three key domains~\cite{airan-alliance}: 

\noindent\textbf{1) AI-for-RAN --} 
This refers to utilizing AI to optimize and enhance the RAN performance.%, motivated by the need to use the limited spectrum efficiently. 
%A classic set of problems in this domain focuses on how the limited spectrum can be used in the most efficient way.
%Such problems were traditionally treated as optimization problems, which were solved through the use of handcrafted heuristics.
%However, such solutions can no longer provide acceptable performance, due to the added complexity that 5G and beyond networks introduce.
The demand for more traffic has led to the introduction of new, higher frequency bands. 
These bands offer more capacity but lower coverage, leading to an increase in the overall tower density. %and a growing asymmetry between macro cells with large coverage and pico/small cells with extra capacity.
Furthermore, new radio resource allocation technologies, like Massive MIMO, see the use of large antenna arrays as a way to further increase the cell capacity.
Assigning users to different bands and managing interference across cells by adjusting scheduling, power control and antenna assignments leads to a search space explosion, which is computationally intractable to manage with conventional optimization methods, making the use of AI a compelling alternative~\cite{bartsiokas2022ml}. 
%AI-based resource management has already shown value in other infrastructures such as datacenters, and holds potential for RAN management.

Similar to radio resource optimization, there exist a whole set of infrastructure optimization problems, caused by the increased 5G complexity, which AI promises to solve.
Telco operators often manage close to 100k RAN sites. 
Predictive maintenance for an infrastructure at that scale (e.g., dealing with hardware issues, software bugs, etc.) is a challenge on its own.
The virtualization of the RAN adds an extra layer of complexity, making the identification and root cause analysis of performance issues far from obvious~\cite{sun2024spotlight}.
Finally, in the context of energy efficiency, %the power consumption of RAN networks worldwide today is estimated to 150TWh annually [link] and is increasing. 
a lot of effort %in platform optimization is 
has been on how to reduce the power consumption of various elements, while maintaining the network coverage and quality, with several AI-based research works showing promising results~\cite{kundu2024towards}.
 

\noindent\textbf{2) AI-and-RAN --}
This domain focuses on the compute sharing (e.g., CPU, GPU) between RAN network functions and AI applications, for efficient utilization of the infrastructure. Typically, virtualized RAN functions utilize the infrastructure lightly (typically $<50\%$ utilization)~\cite{nvidia_vran}, for reasons inherent to the characteristics of the RAN workload.
vRAN servers have to be provisioned for peak capacity, but they typically serve significantly less traffic (e.g., due to the diurnal traffic patterns). 
This inefficiency persists even at times of peak usage due to %fast-scale traffic variations and 
imbalances in the computational demand when processing uplink and downlink traffic~\cite{foukas2021concordia}. 
%For example, the RAN serves traffic in a slotted time division duplex (TDD) fashion, with the uplink traffic being significantly more computationally demanding compared to the downlink.
%This introduces imbalances in the processing load, where the server is more heavily utilized when processing uplink traffic slots compared to downlink.

In contrast to cloud computing, where the sharing of compute resources is commonplace, sharing resources with RAN workloads introduces significant challenges.
The real-time nature of the RAN means that sharing can lead to deadline violations and adversely affect network performance.
%The intricate interactions between the RAN network functions and the infrastructure make hand-crafted solutions sub-optimal.
Several recent proposals have demonstrated how AI can be leveraged to share the infrastructure in both CPUs~\cite{foukas2021concordia} and GPUs~\cite{schiavo2024yinyangran}.


\noindent\textbf{3) AI-on-RAN --}
This domain encompasses use cases that leverage the RAN infrastructure to support AI applications. % that go beyond the telecom boundaries.
A key enabler of such use cases are the open interfaces exposed by the RAN functions, which can allow third-parties to tap into RAN data and/or affect RAN traffic-related decisions, in order to enhance the application capabilities.
One example that falls under this category is localization via sensing.
By leveraging channel state information exposed by the physical layer of the RAN, one can perform user localization, which can be important for several use cases, like asset tracking and self-driving cars~\cite{trevlakis2023localization}.
AI-based techniques leveraging physical layer information can also be employed to provide context-aware security~\cite{chorti2022context}, in consideration of battery-constrained devices. %as a lightweight alternative to existing mechanisms that introduce challenges for battery-constrained devices.
Finally, more traditional AI-based applications, like video analytics could also leverage the interplay with the RAN, to accommodate latency critical use-cases (e.g.,~\cite{zhang2024vulcan}).
